Online Tensor-Based Learning for Multi-Way Data

The online analysis of multi-way data stored in a tensor $\mathcal{X} \in \mathbb{R} ^{I_1 \times \dots \times I_N} $ has become an essential tool for capturing the underlying structures and extracting the sensitive features which can be used to learn a predictive model. However, data distributions often evolve with time and a current predictive model may not be sufficiently representative in the future. Therefore, incrementally updating the tensor-based features and model coefficients are required in such situations. A new efficient tensor-based feature extraction, named NeSGD, is proposed for online $CANDECOMP/PARAFAC$ (CP) decomposition. According to the new features obtained from the resultant matrices of NeSGD, a new criteria is triggered for the updated process of the online predictive model. Experimental evaluation in the field of structural health monitoring using laboratory-based and real-life structural datasets show that our methods provide more accurate results compared with existing online tensor analysis and model learning. The results showed that the proposed methods significantly improved the classification error rates, were able to assimilate the changes in the positive data distribution over time, and maintained a high predictive accuracy in all case studies.

==> ocsvm.tex <==
\section{Preliminaries}
\subsection{One-Class Support Vector Machine}
\label{s:ocsvm}

Given a set of training data $X=\{{x_i}\}_{i=1}^n$, with $n$ being the number of
samples, OCSVM maps these samples into a high dimensional feature space using
a function $\phi$ through  the kernel $K(x_i,x_j) = \phi(x_i)^T \phi(x_j)$.
Then OCSVM learns a decision boundary that maximally separates the
training samples from the origin \cite{scholkopf2001estimating}. The primary
objective of OCSVM   is to optimize  the  following equation:

\vspace{-7mm}
\begin{eqnarray}\label{ocsvm}	
\max_{w,\xi,\rho} -\frac{1}{2} \lVert w \rVert^{2} - \frac{1}{\nu n} \sum_{i=1}^n \xi_i + \rho
\end{eqnarray}
\vspace{-10.5mm}

\begin{eqnarray*}	
	s.t \hspace{2em}  w. \phi(x_i) \geq \rho - \xi_i,\hspace{1em}   \xi_i \geq 0, \hspace{1em}  i = 1, \ldots, n.
\end{eqnarray*}

where $\nu$ $ (0<\nu<1)$ is a user defined parameter  to control the rate of anomalies in the training data, $\xi_i$ are the slack variable, $\phi(x_i)$ is
the kernel matrix and $ w. \phi(x_i) - \rho$ is the separating hyperplane in
the feature space.

The problem  turns  into a dual objective by introducing Lagrange multipliers $
\alpha = \{\alpha_1,\cdots,\alpha_n\}$. This dual optimization problem is solved
using the following  quadratic programming formula \cite{scholkopf2002learning}:
\vspace{-7mm}

\begin{eqnarray}\label{quad}
W=\min_{W(\alpha,\rho)}    \frac{1}{2}\sum_{i}^n \sum_{j}^n\alpha_i\alpha_j \phi(x_i, x_j) + \rho(1 - \sum_{i}^n\alpha_i)
\end{eqnarray}
\vspace{-10mm}
\begin{eqnarray*}
	s.t \hspace{2em} 0 \leq \alpha_i \leq 1,\hspace{1em} \sum_{i=1}^n    \alpha_i =\frac{1}{\nu n}.
\end{eqnarray*}

where $\phi(x_i, x_j)$ is the kernel matrix, $\alpha$ are the Lagrange
multipliers and $\rho$ known as  the bias term.

In the optimal solution,  $\alpha_i = 0$ in the training samples are referred
to as non-support or reserve vectors denoted by \textit{R}. Training vectors
with $\alpha_i=1$  are called non-margin support or error vectors denoted by
\textit{E}, and vectors with  $ 0 < \alpha_i < 1$  are called support vectors
denoted by \textit{S}. The partial derivative of the quadratic optimization problem (defined in
Equation \ref{quad}) with respect to $\alpha_i$,  $\forall i \in S$,  is then
used as a decision function to calculate  the  score for  a new incoming
sample:
\vspace{-3mm}
\begin{eqnarray}\label{dv2}
g(x_i) = \frac{\partial w}{\partial \alpha_i} =  \sum_{j}\alpha_i \phi(x_i, x_{j})-\rho.
\end{eqnarray}
%\begin{eqnarray}\label{b}
%\frac{\partial w}{\partial \rho} =   \sum_{i=1}^{n}\alpha_i-1=0
%\end{eqnarray}

\vspace{-3mm}
The achieved OCSVM solution must always satisfy the constraints from the KKT
conditions, which are described in Equation~\ref{kkt}.\vspace{-4mm}

\begin{eqnarray}\label{kkt}
g(x) = \Bigg\{\begin{tabular}{ccc}
$\geq$ 0 &   & $\alpha_i=0$ \\
= 0 &  & $ 0 < \alpha_i < 1$\\%\frac{1}{\nu n}$\\
$<$ 0  &   &$   \alpha_i  = 1 $%\frac{1}{\nu n}$
\end{tabular}
\end{eqnarray}

The OCSVM uses Equation \ref{df}  to identify whether a new incoming point
belongs to the positive class when returning a positive value, and vice versa if
it generates a negative value.\vspace{-7mm}

\begin{eqnarray}\label{df}
f(x_i) = sgn(g(x_i))
\end{eqnarray}




